Ego2X: Contact-aware Transfer from Egocentric Human Data to Any Robot

Embodied models depend on real interaction data, yet collecting it on physical robots is slow and labor-intensive. Recent ego-to-robot pipelines retarget first-person view human videos to robot data via transferring hand and arm motion. They judge fidelity mainly by visual appearance. However, trajectories often fail in terms of physics: fingers hover beside objects, and grippers close on empty space. We argue that how the object moves and the contacts that drive the motion count. Thus, we present Ego2X, an object-centric framework that converts monocular egocentric video into physically executable robot data across dexterous hands and parallel grippers. Ego2X centers on CORE (Contact-centric Object-interaction REpresentation), which records each contact on the object by its surface anchor, as well as relative force, grasp mode, and interaction state. Throughout the pipeline, CORE corrects hand-object drift via object-relative constraints, steers inverse kinematics toward contacts the robot must realize, and preserves held objects during arm erasure and robot compositing. On HOT3D, contact-driven correction reduces in-contact hand depth error by 33.7%, while on EgoDex, contact-driven retargeting realizes 62.9% of annotated contacts, surpassing the official HuRo pipeline (27.9%). In RoboTwin 2.0, post-training X-VLA on Ego2X episodes alone, without simulator demonstrations, raises task success rate from 40.5% zero-shot to 67.0% across 200 paired scenes. We will publicly release our conversion pipeline and CORE-annotated dataset for dexterous hands and parallel grippers.

==> tables/tab_conversion.tex <==
\begin{table}[t]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.94}
\setlength{\tabcolsep}{1.8pt}
\caption{\textbf{Closed-loop demonstration yield in RoboTwin~2.0.} Top: episodes passing the official simulator task check from identical pools ($52$ matched \emph{Bread in basket} episodes, $70$ expanded; $53$ \emph{Bell on scale} specifications across $24$ takes, sign test $23{:}0{:}1$, Holm $p=4.8{\times}10^{-7}$). Bottom: Phase-1 candidate feasibility (motion planning, joint legality, and simulator check across $348$ regenerated layouts per arm).}
\label{tab:conversion}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}llcc@{}}
\toprule
Task / Stage & Pipeline & Passing $\uparrow$ & Rate / $\Delta$ \\
\midrule
\multirow{2}{*}{Bread ($52$)} & HuRo~\cite{huro} / E2R~\cite{ego2robot} & 1 / 1 & $1.9\%$ / $1.9\%$ \\
                              & Ego2X (matched / exp.) & \textbf{31} (70) & \textbf{59.6\%} \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Bell on\\scale ($53$)\end{tabular}} & HuRo~\cite{huro} / E2R~\cite{ego2robot} & 0 / 0 & $0.0\%$ / $0.0\%$ \\
                                      & Ego2X (all / zero-retry) & \textbf{45 / 40} & \textbf{84.9} / 75.5\% \\
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Phase-1 cand.\\feas.\ ($348$)\end{tabular}} & E2R $+$ our protocol & 101 & 29.0\% ($p{=}0.019$) \\
                                 & HuRo $+$ our protocol & 124 & 35.6\% (n.s.) \\
                                 & Ego2X (ours) & \textbf{135} & \textbf{38.8\%} \\
\bottomrule
\end{tabular*}
\vspace{0.3em}
\end{table}


==> tables/tab_embodiments.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{1.7pt}
\caption{\textbf{One CORE record, many embodiments.} Five grippers on $14$ shared episodes under a common pinch-point TCP; rate-retimed ALLEX ($\le 7.5$\,rad/s) on the $81$ released episodes ($0.933$ pooled over $5{,}171$ slots).}
\label{tab:embodiments}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcccc@{}}
\toprule
Embodiment & EEF Real.\ $\uparrow$ & 95\% CI & Pen.\ $\downarrow$ & Arm IK / Free \\
\midrule
Panda + 2F-85    & 0.809 & [0.621, 0.914] & \textbf{0.020} & 0.457 / 0.592 \\
ARX5 (Aloha)     & 0.810 & [0.625, 0.909] & 0.026 & 0.620 / 0.719 \\
Franka Hand      & 0.797 & [0.609, 0.902] & 0.024 & 0.558 / 0.765 \\
UR5 + WSG50      & 0.796 & [0.606, 0.901] & 0.026 & \textbf{0.695} / 0.751 \\
Piper            & \textbf{0.820} & [0.635, 0.918] & 0.027 & 0.032 / \textbf{0.839} \\
\midrule
ALLEX (released) & \textbf{0.902} & [0.846, 0.946] & 0.025 & wrist driven \\
\bottomrule
\end{tabular*}
\vspace{-0.5em}
\end{table}


==> tables/tab_ik_velocity.tex <==
\begin{table}[t]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.94}
\setlength{\tabcolsep}{2.2pt}
\caption{\textbf{Equal-caliber joint-rate distribution ($\max_j |\dot{q}_j|$).} Evaluated across $22$ shared joints on $8{,}104$ frames ($79$ EgoDex takes). $^{\ddagger}$Step-limiter saturation at $7.5$\,rad/s ($0.0\%$ true excursions); $^{\dagger}$unbounded excursions.}
\label{tab:ik_velocity}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
\toprule
Method & Med. & $p_{90}$ & $p_{99}$ & Max & ${>}6$ (\%) & ${>}7.5$ (\%) \\
\midrule
Ours (\texttt{CARD}, Eq.~\ref{eq:ik}) & 2.59 & 4.78 & 7.50 & 7.50 & 7.11 & 2.64$^{\ddagger}$ \\
Ours, wrist following (\texttt{wf}) & 1.47 & 2.51 & 7.50 & 7.50 & 1.92 & 0.83$^{\ddagger}$ \\
HuRo stage-8~\cite{huro} & 1.05 & 2.45 & 7.73 & 63.92 & \textbf{1.48} & 1.04$^{\dagger}$ \\
\bottomrule
\end{tabular*}
\vspace{0.3em}
\end{table}


==> tables/tab_vs_huro.tex <==
\begin{table}[t]
\centering
\scriptsize
\renewcommand{\arraystretch}{0.94}
\caption{\textbf{Same-take conversion comparison against HuRo.} Both methods convert the identical EgoDex takes; contact realization and pseudo-signed frame penetration ($<-1$\,mm) are evaluated on the shared 73-take $\texttt{GEOM}{\cap}\texttt{HC}$ roster ($8{,}573$ slots, \cref{tab:ik_dex}).}
\label{tab:vs_huro}
\setlength{\tabcolsep}{2.0pt}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lll@{}}
\toprule
Exported field / metric & HuRo~\cite{huro} & Ego2X (ours) \\
\midrule
Object mesh, pose \& trust & absent & per frame, with SDF $\phi_o$ \\
Contacts, modes \& forces & absent & object-frame $\mathbf{c}_{t,k}$ \\
Interaction state $s_{t,k}$ & task label & per frame, 5 states \\
Camera \& quality masks & absent & $\mathbf{K}$, poses, layer masks \\
Parallel-gripper stream & unavailable & 5 grippers (6-DoF TCP + width) \\
Held-object pixels & no render & preserved + de-skinned \\
\midrule
Contact realiz.\ ($\texttt{GEOM}{\cap}\texttt{HC}$)$\uparrow$ & $0.708$ & $\mathbf{0.895}$ ($+22.7$\,pp paired) \\
Penetrating frames (SDF)$\downarrow$ & $0.041$ & $0.044$ ($p{=}0.393$) \\
\bottomrule
\end{tabular*}
\end{table}

